Cordial Miners: Fast and Efficient Consensus for Every Eventuality

Cordial Miners are a family of efficient Byzantine Atomic Broadcast protocols, with instances for asynchrony and eventual synchrony. They improve the latency of state-of-the-art DAG-based protocols by almost 2X and achieve optimal good-case complexity of O(n) by forgoing Reliable Broadcast as a building block. Rather, Cordial Miners use the blocklace -- a partially-ordered counterpart of the totally-ordered blockchain data structure -- to implement the three algorithmic components of consensus: Dissemination, equivocation-exclusion, and ordering.

==> Code/optimization.tex <==
% \begin{figure}[t]
\begin{algorithm*}[t]
	\caption{\textbf{\sys: Optimization for ES.} Code for miner $p$.}
	\label{alg:optimization}
%	\small
%        \vspace{-1em}
	% \begin{flushleft}
        % \noindent\textbf{\ref{alg:protocols}.1 Procedures for Asynchrony}
        % \end{flushleft}
 %       \vspace{-1em}
      \begin{algorithmic}[1]  \scalefont{0.8}
   
        \Procedure{$\textit{es\_timeout()}$}{}: \label{alg:completed-es-opt}

        
        \State \Return $\max~ r : \textit{cordial\_round}(r) ~\wedge$ \Comment{Last cordial round, \cref{alg:cordial-round}}

        \State (($r \text{ mod } w = 0 \implies$ \Comment{First round of the wave, leader is included in the round.}
         \State $\exists b \in \textit{blocklace}: (\textit{leader}(r) = b.\textit{creator})~ \wedge$
    
         \State $( (r \text{ mod } w = 1 \implies$ \Comment{Second round of the wave, round $r-1$ leader is ratified by round $r$ blocks} \label{alg:odd-round}
         \State $\exists b \in \textit{blocklace}: (\textit{leader}(r-1) = b.\textit{creator}~ \wedge$ 
          $\textit{ratifies}(\textit{blocklace\_prefix}(r),b)))~ \wedge$ 
           \label{alg:ratified-es}   
        
       \State $( (r \text{ mod } w = 2 \implies$ \Comment{Third round, round $r-2$ leader is super-ratified by $r$ blocks} \label{alg:second-round}
         \State $\exists b \in \textit{blocklace}: (\textit{leader}(r-2) = b.\textit{creator}~ \wedge$ 
          $\textit{super-ratifies}(\textit{blocklace\_prefix}(r),b)))$ 
           \label{alg:ratified2-es} 
          
        \State  $\vee~  \textit{timeout})$  \label{alg:timeout-es}    \Comment{Or timeout occurred. \textit{timeout} is measured from when round $r$ is cordial. This is $p$'s estimation of $\Delta$.}
        \EndProcedure
	

		\alglinenoPush{counter}
  \end{algorithmic}	
	% \end{changemargin}
\end{algorithm*}
% \vspace{-2em}
% \end{figure}

